FastDiagP: An Algorithm for Parallelized Direct Diagnosis

Constraint-based applications attempt to identify a solution that meets all defined user requirements. If the requirements are inconsistent with the underlying constraint set, algorithms that compute diagnoses for inconsistent constraints should be implemented to help users resolve the "no solution could be found" dilemma. FastDiag is a typical direct diagnosis algorithm that supports diagnosis calculation without predetermining conflicts. However, this approach faces runtime performance issues, especially when analyzing complex and large-scale knowledge bases. In this paper, we propose a novel algorithm, so-called FastDiagP, which is based on the idea of speculative programming. This algorithm extends FastDiag by integrating a parallelization mechanism that anticipates and pre-calculates consistency checks requested by FastDiag. This mechanism helps to provide consistency checks with fast answers and boosts the algorithm's runtime performance. The performance improvements of our proposed algorithm have been shown through empirical results using the Linux-2.6.3.33 configuration knowledge base.

==> tex/fastdiag.tex <==
% \begin{algorithm}
% \caption{\textsc{FastDiag}$(C, B): \Delta$}
% \small
% \begin{algorithmic}[1]\label{alg:fastdiag}
% \IF{$C=\emptyset$ or \textsc{Consistent}$(B \cup C)$}
% % \STATE \emph{write}('consistent')
% \STATE \emph{return}($\emptyset$)
% % \ELSIF{}
% % \STATE \emph{return}($\emptyset$)
% \ELSE
% \STATE \emph{return}($C \setminus \textsc{FD}(C,B,\emptyset)$)
% \ENDIF
% \end{algorithmic}
% \end{algorithm}

==> tex/fd.tex <==
% \begin{algorithm}
% \caption{$\textsc{FD}(C=\{c_1..c_n\},B,\rho): \Omega$}
% \small
% \begin{algorithmic}[1] \label{alg:fd}
% \IF{$\rho \neq \emptyset$ and $\textsc{Consistent}(B \cup C)$}
% \STATE \emph{return}($C$)
% \ENDIF
% \IF{$|C|=1$}
% \STATE \emph{return}($\emptyset$)
% \ENDIF
% \STATE \textsc{Split}$(C, C_l, C_r)$
% % \STATE $k=\lfloor\frac{n}{2}\rfloor$
% % \STATE $C_l \leftarrow c_1 \ldots c_{k}; C_r \leftarrow c_{k+1} \ldots c_{n}$
% \STATE $\Omega_2 \leftarrow \textsc{FD}(C_l,B,C_r)$
% \STATE $\Omega_1 \leftarrow \textsc{FD}(C_r,B \cup \Omega_2,C_l \setminus \Omega_2)$
% \STATE \emph{return}($\Omega_1 \cup \Omega_2$)
% \end{algorithmic}
% \end{algorithm}

==> tex/isconsistent.tex <==
% \begin{algorithm}
% \caption{\textsc{Consistent}$(C, B, \rho): Boolean$}
% \small
% \begin{algorithmic}[1]\label{alg:isconsistent}
% % \IF{$C=\emptyset$}
% % \STATE \emph{return}$(True)$
% % \ENDIF
% \IF{$\neg \textsc{ExistCC}(B \cup C)$}
% \STATE \textsc{LookAhead}$(C, B, \{ \rho \})$
% \ENDIF
% \STATE \emph{return} \textsc{LookUp}$(B \cup C)$
% \end{algorithmic}
% \end{algorithm}

==> tex/lookahead.tex <==
% \begin{algorithm}[t]
% \caption{\\\textsc{LookAhead}$(C, B, \phi= \{\{\phi_1\}..\{\phi_p\}\})$}
% \small
% \begin{algorithmic}[1]\label{alg:lookahead}
% \IF{$curGCC < maxGCC$}
%     \IF{$\neg \textsc{ExistCC}(B \cup C)$}
%         \STATE $curGCC \leftarrow curGCC + 1$
%         \STATE \textsc{AddCC}($B \cup C$)
%     \ENDIF
    
%     \STATE \textcolor{teal}{\{$B \cup C$ \textit{assumed consistent}\}}
%     \IF[case 1.1]{$|\phi| > 1 \land |\phi_1| = 1 \land \textsc{ExistCC}(B \cup C \cup \phi_1)$}
%         \STATE \textsc{Split}$(\phi_2, \phi_{2l}, \phi_{2r})$
%         \STATE \textsc{LookAhead}$(\phi_{2l}, B \cup C, \phi_{2r} \cup  (\phi \setminus \{ \phi_1, \phi_2 \}))$
%     \ELSIF[case 1.2]{$\phi \neq \emptyset \land |\phi_1| = 1$}
%         \STATE \textsc{LookAhead}$(\phi_1, B \cup C, \phi \setminus \phi_1)$
%     \ELSIF[case 1.3]{$\phi \neq \emptyset \land |\phi_1| > 1$}
%         \STATE \textsc{Split}$(\phi_1, \phi_{1l}, \phi_{1r})$
%         \STATE \textsc{LookAhead}$(\phi_{1l}, B \cup C, \phi_{1r} \cup  (\phi \setminus \phi_1))$
%     \ENDIF
    
%     \STATE \textcolor{teal}{\{$B \cup C$ \textit{assumed inconsistent}\}}
%     \IF[case 2.1]{$|C| > 1$}
%         \STATE \textsc{Split}$(C, C_l, C_r)$
%         \STATE \textsc{LookAhead}$(C_l, B, C_r \cup \phi)$
%     \ELSIF[case 2.2]{$|C| = 1 \land |\phi_1| = 1$}
%         \STATE \textsc{LookAhead}$(\phi_1, B, \phi \setminus \phi_1)$
%     \ELSIF[case 2.3]{$|C| = 1 \land |\phi_1| > 1$}
%         \STATE \textsc{Split}$(\phi_1, \phi_{1l}, \phi_{1r})$
%         \STATE \textsc{LookAhead}$(\phi_{1l}, B, \phi_{1r} \cup  (\phi \setminus \phi_1))$
%     \ENDIF
% \ENDIF
% \end{algorithmic}
% \end{algorithm}

==> tex/table-LookUp.tex <==
% \begin{table}[ht]
% \small
% \caption{A \textsc{LookUp} table created in our working example, including part of consistency checks generated by \textsc{AddCC} in the \textsc{LookAhead} function (see \textit{Figure \ref{fig:fastdiagp-ex-tree}}) and executed in parallel. The `--' entries indicate that the corresponding consistency checks are still ongoing or have not been started.} 
% \centering 
% \begin{tabular}{|l|l|c|c|c|}
% \hline
% node-id & constraint set 	& consistent   
% \tabularnewline
% \hline
% $1$ & $\{C_{KB} \cup \{c_{10} \twodots c_{13}\}\}$ & $false$
% \tabularnewline
% \hline
% $1.2$ & $\{C_{KB} \cup \{c_{10},c_{11}\}\}$ & $false$
% \tabularnewline
% \hline
% $1.2.1$ & $\{C_{KB} \cup \{c_{10},c_{11},c_{12}\}\}$ & --
% \tabularnewline
% \hline
% $1.2.1.2$ & $\{C_{KB} \cup \{c_{10},c_{11},c_{13}\}\}$ & --
% \tabularnewline
% \hline
% $1.2.2$ & $\{C_{KB} \cup \{c_{10}\}\}$ & $true$
% \tabularnewline
% \hline
% % $1.2.2.1$ & $\{C_{KB} \cup \{c_{10},c_{12}\}\}$	& --
% % \tabularnewline
% % \hline
% % $1.2.2.1.1$ & $\{C_{KB} \cup \{c_{10},c_{12},c_{13}\}\}$	& --
% % \tabularnewline
% % \hline
% % $1.2.2.1.2$ & $\{C_{KB} \cup \{c_{10},c_{13}\}\}$	& --
% % \tabularnewline
% % \hline
% % $1.2.2.2$ & $\{C_{KB} \cup \{c_{11}\}\}$	& --
% % \tabularnewline
% % \hline
% % $1.2.2.2.1$ & $\{C_{KB} \cup \{c_{11},c_{12}\}\}$	& --
% % \tabularnewline
% % \hline
% \end{tabular} 
% \label{tab:Lookup-table}
% \end{table}

==> tex/table-constraints.tex <==
% \begin{table}[!ht]
% \small
%     \begin{center}
%     {\caption{Constraints in $C_{KB} = \{c_0 \twodots c_9\}$ derived from our simplified configuration knowledge base, $C_R = \{c_{10} \twodots c_{13}\}$ is a set of user requirements.}%The constraint $c_0:Smartwatch=t$ is regarded as \emph{root constraint} that is used to avoid the derivation of (irrelevant) empty conﬁgurations.}

%     \label{table:ex_kb}}
%     \begin{tabular}{x{0.6cm}y{4cm}x{0.7cm}y{1.9cm}}
%     \hline
%           & \multicolumn{3}{l}{\textbf{CSP representation}}\tabularnewline
%     \hline
%           & \multicolumn{3}{l}{\textbf{Constraints in the knowledge base} - $C_{KB}$}\tabularnewline
%     $c_0$ & \multicolumn{3}{l}{$Smartwatch=t$}\tabularnewline
%     $c_1$ & \multicolumn{3}{l}{$Smartwatch \leftrightarrow Connector$} \tabularnewline
%     $c_2$ & \multicolumn{3}{l}{$Smartwatch \leftrightarrow Screen$} \tabularnewline
%     $c_3$ & \multicolumn{3}{l}{$Camera \rightarrow Smartwatch$} \tabularnewline
%     $c_4$ & \multicolumn{3}{l}{$Compass \rightarrow Smartwatch$} \tabularnewline
%     $c_5$ & \multicolumn{3}{l}{$Connector \leftrightarrow (GPS \vee Cellular \vee Wifi \vee Bluetooth)$} \tabularnewline
%     % $c_6$ & $(Analog \leftrightarrow \neg High$ $Resolution \wedge \neg E$-$ink \wedge Screen)$ \\
%     % & $\wedge (High$ $Resolution \leftrightarrow \neg Analog \wedge \neg E$-$ink \wedge Screen)$ \\
%     % & $\wedge (E$-$ink \leftrightarrow \neg Analog \wedge \neg High$ $Resolution \wedge Screen)$ \\
%     $c_6$ & \multicolumn{3}{l}{$Screen \leftrightarrow xor(Analog, High$ $Resolution, E$-$ink)$} \tabularnewline
%     $c_7$ & \multicolumn{3}{l}{$Camera \rightarrow High$ $Resolution$} \tabularnewline
%     $c_8$ & \multicolumn{3}{l}{$Compass \rightarrow GPS$} \tabularnewline
%     $c_9$ & \multicolumn{3}{l}{$\neg(Cellular \wedge Analog)$} \tabularnewline
%     \hline
%     & \multicolumn{3}{l}{\textbf{User requirements} - $C_R$}\tabularnewline
%     $c_{10}$ & \hspace{6pt}$Cellular=t$ & $c_{12}$ & $Compass=t$\tabularnewline
%     $c_{11}$ & \hspace{6pt}$Analog=t$ & $c_{13}$ & $GPS=f$\tabularnewline
%     % $c_{12}$ & $Compass=t$\tabularnewline
%     % $c_{13}$ & $Camera=t$\\ 
%     % $c_{13}$ & $GPS=f$\tabularnewline
%     % $c_{15}$ & $Wifi=t$\\ 
%     % $c_{16}$ & $Bluetooth=t$\\
%     \hline
%     \end{tabular}
%     \end{center}
% \end{table}

==> tex/table-followsets.tex <==
% \begin{table*}
% \caption{Options of the \textsc{LookAhead}'s parameters with regard to the assumption about the consistency of $B \cup C$ and the current value of $C$ and $\Delta$.}
% \label{tab:follow-sets}
% \centering \small
% \begin{tabular}{|l|l|c|c|c|}
% \hline
%  & & \multicolumn{3}{c|}{\textsc{Follow Sets}}  
% \tabularnewline
% \cline{3-5}
% \textsc{Assumption of $B \cup C$} & \textsc{Condition} & $C$ & $B$ & $\Delta$ \tabularnewline
% \hline
% \multirow{3}{*}{$B \cup C$ \emph{assumed inconsistent}} & $|C| > 1$ & $C_l$ & $B$ &  $C_r \cup \Delta$ \tabularnewline
% \cline{2-5}
% & $|C| = 1 \land |\Delta_1| = 1$ & $\Delta_1$ & $B$ &  $\Delta \setminus \Delta_1$ \tabularnewline
% \cline{2-5}
% & $|C| = 1 \land |\Delta_1| > 1$ & $\Delta_{1l}$ & $B$ & $\Delta_{1r} \cup  (\Delta \setminus \Delta_1)$ \tabularnewline
% \hline
% \multirow{3}{*}{$B \cup C$ \emph{assumed consistent}} & $|\Delta| > 1 \land \textsc{ExistConsistencyCheck}(B \cup C \cup \Delta_1)$ & $\Delta_{2l}$ & $B \cup C$  & $\Delta_{2r} \cup  (\Delta \setminus \{ \Delta_1, \Delta_2 \})$ \tabularnewline
% \cline{2-5}
% & $\Delta \neq \emptyset \land |\Delta_1| = 1$ & $\Delta_1$  & $B \cup C$ & $\Delta \setminus \Delta_1$ \tabularnewline
% \cline{2-5}
% & $\Delta \neq \emptyset \land |\Delta_1| > 1$ & $\Delta_{1l}$ & $B \cup C$  & $\Delta_{1r} \cup  (\Delta \setminus \Delta_1)$  \tabularnewline
% \hline
% \end{tabular} 
% \vspace{10pt}
% \end{table*}

==> tex/table-linux.tex <==
% \begin{table}[h]
% \caption{Characteristics of the \emph{Linux-2.6.33.3} feature model.}
% \label{tab:linux} 
% \centering 
% \begin{tabular}{|l|r|}
% \hline
% \#features & $6,467$ \tabularnewline  \hline
% \#relationships & $6,322$ \tabularnewline  \hline
% %\%CTC ratio & $54.7\%$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#mandatory} & $244$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#optional} & $6,037$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#alternative} & $39$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#or} & $2$ \tabularnewline  \hline
% \#cross-tree constraints & $7,650$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#requires} & $7,108$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#excludes} & $205$ \tabularnewline  \hline
% \multicolumn{1}{|r|}{\#3 CNF} & $337$ \tabularnewline  \hline
% \end{tabular}
% \end{table}

